Chain-of-Thought Matters: Improving Long-Context Language Models with Reasoning Path Supervision

Recent advances in Large Language Models (LLMs) have highlighted the challenge of handling long-context tasks, where models need to reason over extensive input contexts to aggregate target information. While Chain-of-Thought (CoT) prompting has shown promise for multi-step reasoning, its effectiveness for long-context scenarios remains underexplored. Through systematic investigation across diverse tasks, we demonstrate that CoT's benefits generalize across most long-context scenarios and amplify with increasing context length. Motivated by this critical observation, we propose LongRePS, a process-supervised framework that teaches models to generate high-quality reasoning paths for enhanced long-context performance. Our framework incorporates a self-sampling mechanism to bootstrap reasoning paths and a novel quality assessment protocol specifically designed for long-context scenarios. Experimental results on various long-context benchmarks demonstrate the effectiveness of our approach, achieving significant improvements over outcome supervision baselines on both in-domain tasks (+13.6/+3.8 points for LLaMA/Qwen on MuSiQue) and cross-domain generalization (+9.3/+8.1 points on average across diverse QA tasks). Our code, data and trained models are made public to facilitate future research.

==> backup.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|cccccc}
\toprule
    \textbf{Model}  & \textbf{Method} & \textbf{MuSiQue*}  & \textbf{HotpotQA} & \textbf{MultiFieldQA-En}  & \textbf{Qasper}  & \textbf{2WikiMQA}  & \textbf{Avg.}               \\
    \midrule
    \multirow{2}{*}{\textit{Qwen-2.5-7B-Base}} & \quad + ORM & 49.15           & \textbf{58.13}              &  43.16              & 29.71              & 41.18  &   44.26 \\
    &  \quad + \textbf{Ours} & \textbf{47.6} & 58.06 & \textbf{44.68} & \textbf{38.13} & \textbf{55.49} &\textbf{48.79} \\
    \midrule
    \multirow{2}{*}{\textit{Llama-3.1-8B-Base}} & \quad + ORM & 47.01           & 50.02              &  \textbf{44.44}              & 32.06              & 37.08  &   42.12 \\
    &  \quad + \textbf{Ours} & \textbf{52.62} & \textbf{54.45} & 43.84 & \textbf{33.19} & \textbf{51.62} & \textbf{47.14} \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison of different models and methods on various datasets. The \textsc{ORM} method represents the original base models without any CoT enhancement, while \textsc{Ours} represents the proposed two-stage training framework.}
\label{tab:main_results} 
\end{table*}

\begin{table*}[htbp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lccccccccc}
    \toprule
        \multirow{2.5}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{LongBenchV1}} & \multicolumn{3}{c}{\textbf{LongBenchV2}} & \multirow{2.5}{*}{\textbf{Avg.}} \\
        \cmidrule(lr){2-6} \cmidrule(lr){7-9}
        & \textbf{MuSiQue*} & \textbf{HPQA} & \textbf{MFQA} & \textbf{Qasper} & \textbf{2WMQA} & \textbf{SQA} & \textbf{MQA} & \textbf{LICL} & \\
        \midrule
        \textit{Llama-3.1-8B-Warmup}\\
        \midrule
        \quad + ORM & 47.01 & 50.02 & 44.44 & 32.06 & 37.08 & 13.41 & 9.57 &18.18 & 31.47 \\
        \quad + \textbf{Ours} & 53.98 & 54.64 & 42.85 & 34.51 & 54.59 & 20.73 & 25.22 &18.18 & 38.08 \\
        \quad + \textbf{Ours} +\textbf{Reject Sampling} & 57.04 & 54.66 & 44.58 &36.38 &57.27 &25.61 &25.22 &24.24 &40.62 \\
        \quad + \textbf{Ours} + \textbf{Gpt-4o Sampling} & 56.95 & 60.73 &45.59 &39.62 &63.67 \\
        \\ \midrule
        \textit{Qwen-2.5-7B-Warmup}\\
        \midrule
        \quad + ORM & 49.15 & 58.13 & 43.16 & 29.71 & 41.18 & 12.20 & 8.70 & 12.12 &31.79 \\
        \quad + \textbf{Ours} & 49.78 & 54.40 & 44.38 & 38.14 & 61.85 & 28.05 &30.43 & 33.33&42.54 \\
        \quad + \textbf{Ours} +\textbf{Reject Sampling} \\
        \quad + \textbf{Ours} + \textbf{Gpt-4o Sampling}
         \\
    \bottomrule
\end{tabular}
\caption{Performance comparison of different models and methods on various datasets. The \textsc{ORM} method represents the original base models without any CoT enhancement, while \textsc{Ours} represents the proposed two-stage training framework. \textit{HPQA}, \textit{MFQA}, \textit{2WMQA} is short for HotpotQA, MultiFieldQA, 2WikiMQA respectively.}
\label{tab:main_results} 
\end{table*}
